Reinventing High Performance Computing: Challenges and Opportunities

The world of computing is in rapid transition, now dominated by a world of smartphones and cloud services, with profound implications for the future of advanced scientific computing. Simply put, high-performance computing (HPC) is at an important inflection point. For the last 60 years, the world's fastest supercomputers were almost exclusively produced in the United States on behalf of scientific research in the national laboratories. Change is now in the wind. While costs now stretch the limits of U.S. government funding for advanced computing, Japan and China are now leaders in the bespoke HPC systems funded by government mandates. Meanwhile, the global semiconductor shortage and political battles surrounding fabrication facilities affect everyone. However, another, perhaps even deeper, fundamental change has occurred. The major cloud vendors have invested in global networks of massive scale systems that dwarf today's HPC systems. Driven by the computing demands of AI, these cloud systems are increasingly built using custom semiconductors, reducing the financial leverage of traditional computing vendors. These cloud systems are now breaking barriers in game playing and computer vision, reshaping how we think about the nature of scientific computation. Building the next generation of leading edge HPC systems will require rethinking many fundamentals and historical approaches by embracing end-to-end co-design; custom hardware configurations and packaging; large-scale prototyping, as was common thirty years ago; and collaborative partnerships with the dominant computing ecosystem companies, smartphone, and cloud computing vendors.

==> Cloudservices.tex <==
\section{Rich Cloud Services}
\label{sec:services}
%
The early cloud data centers were built to support specific tasks such as email and web search. While they were large for their time, they are dwarfed by the current deployments.  The driving force of this explosive growth was the realization that the data center itself was a consumer product.  In 2006 Amazon launched its ''Simple Storage Service'' (s3) to allow anybody with a credit card to store data ''in the cloud.''  A few months later they introduced the ''Elastic Compute Cloud'' (ec2) that was built upon virtual machine technology. This proved to be a boon for start-up companies who need an on-line presence but lacked the resources to build a data center.  Ec2 could automatically expand as their business grew.  Amazon Web Services, as the new division of Amazon was called, made s3 and ec2 more valuable by releasing relational database services and DynamoDB a ''noSQL'' on-line database service. By 2008 Microsoft was busy working on their own cloud services.  Microsoft Azure was announced in 2008 and released in 2010 with basic cloud storage and virtual machine capabilities.   While Google already had a very large data center deployment and numerous powerful internally developed and used cloud services the first public services was called AppEngine and released in 2011.  

An explosion in cloud capabilities followed these early services. In addition,  the growing movement of open source software was driving dramatic changes in the industry. Open source cloud platforms like Eucalyptus \cite{eucalyptus} and OpenStack \cite{openstack} allowed others to start building cloud platforms. A fundamental development in cloud service software architecture was the use of microservices. This was a way to break massive-scale, multiuser cloud applications into many small interdependent service units to allow applications to scale and be upgraded while running uninterrupted.  Google released their Kubernetes microservice framework \cite{kubernetes} to the open source community in 2014. More formally Kubernetes is a container orchestration service that supports software packaged with tools like the open-source Docker container system.  Together Kubernetes, Docker and a few other systems have become the foundation of the ''Cloud Native Software'' movement which is now supported by all major cloud vendors. (Versions of Kubernetes and container services are now supported on several supercomputer platforms \cite{}.) Another important addition to the software stack has been the development of serverless computing.  This allows computation to be fully abstracted away from the underlying infrastructure thus allowing computation to migrate between the cloud and edge computing devices.  

While cloud native software frameworks have become standard tools for developers, they are not the top of the software stack.  Enterprise customers were most interested services to help them better serve their customers.  As mentioned above, for the cloud companies the differentiating services has become machine learning and other AI capabilities such as voice-to-text and test-to-speech, document analysis, fraud detection, recommendation service, image and video analysis, demand forecasting.  IBM has introduced the Watson AI service platform on top of its cloud.  Amazon released its SageMaker AI toolkit and a host of ready to use AI tools. Google Cloud offers a variety of cloud AI services backed up by Tensor Processing Units.   Similar tools are offered by the Microsoft Azure Cognitive Service and  ML workspaces development environment. Finally, Tensorflow from Google and Torch from Meta have become the open source industry standard tools for AI development.  

The cloud push for AI did not stop there. All of cloud vendors began buying or partnering with the most advanced AI start-ups.  Google acquired DeepMind in the U.K. in 2014.  Microsoft partnered with OpenAI in 2019. Meta (Facebook) and Amazon have each acquired several smaller AI startups. DeepMind and OpenAi have been using of their parent/partner cloud companies to build massive semi-supervised language models that are changing the game for AI.  The deep learning methods developed by these companies are changing the course of computational science.  The work by DeepMind on protein folding and the University of Washington with help from Microsoft Azure on protein-protein interaction are changing bio-science.  In other areas,  OpenAI is showing deep learning can solve challenging Math Olympiad problems \cite{}. In astrophysics deep learning is being used to classify galaxies\cite{}, generative adversarial networks (GANS) \cite{gan} have been harness to understand ground water flow in superfund sites \cite{},  deep neural networks have been trained to help design non-photonic structures \cite{}.  Even the flagship conference of supercomputing sc2021 had over 20 papers on neural networks in its highly selective program.

%Training Deep Neural Networks for the Inverse Design of Nanophotonic Structures https://pubs.acs.org/doi/10.1021/acs.jctc.8b00636

%Highly-scalable, physics-informed GANs for learning solutions of stochastic PDEs”, arXiv:1910.13444v1.

Supercomputing is clearly now a part of cloud computing. This fact is now clear from the announcement that Meta is building an AI supercomputer. When complete in 2022 it will have 2000 NVIDIA dgx A100 nodes.\cite{}  Microsoft Azure has added a Cray supercomputer to its global network.  


